Spectral Methods for Quantum Optimal Control: Artificial Boundary Conditions

The problem of quantum state preparation is one of the main challenges in achieving the quantum advantage. Furthermore, classically, for multi-level problems, our ability to solve the corresponding quantum optimal control problems is rather limited. The ability of the latter to feed into the former may result in significant progress in quantum computing. To address this challenge, we propose a formulation of quantum optimal control that makes use of artificial boundary conditions for the Schr\"odinger equation in combination with spectral methods. The resulting formulations are well suited for investigating periodic potentials and lend themselves to direct numerical treatment using conventional methods for bounded domains.

==> old/removed.tex <==

\subsection{Application: Quantum Image Processing}


Quantum Image Processing \cite{VenegasAndraca2003, Le2010} is an emerging field of Quantum Information Science that holds the promise of considerable speedups over classical methods such as Deep Neural Networks (DNNs) for certain but common task such as edge detection \cite{Zhang2014,yao2017quantum}. For example, Ref. \cite{Zhang2014} a quantum image edge extraction algorithm, QSobel, that can, in principle, extract edges of a quantum image with $2^n\times 2^n$ pixels in $\mathcal{O}(n^2)$ time, offering an exponential speedup compared to classical edge extraction algorithms. There, the state to be enconded is represented as
\begin{align}
    \ket{I(\theta)} & = \sum_{\rm{pixels}}\ket{\text{color}}\ket{\text{pixel position}} \\
                    &=\frac{1}{2^n} \sum_{i=0}^{2^{2 n}-1}\left(\cos \theta_i|0\rangle+\sin \theta_i|1\rangle\right)|i\rangle,
\end{align}
where the color of the $i$-th pixel is encoded as $\cos \theta_i\ket{0}+\sin \theta_i \ket{1}$, while the position of the $i$-th pixel is represented as a state $\ket{i}$.


However, the difficulty lies in the encoding of the images to the initial quantum states to be processed. 

